Executable Refinement Types

This dissertation introduces executable refinement types, which refine structural types by semi-decidable predicates, and establishes their metatheory and accompanying implementation techniques. These results are useful for undecidable type systems in general. Particular contributions include: (1) Type soundness and a logical relation for extensional equivalence for executable refinement types (though type checking is undecidable); (2) hybrid type checking for executable refinement types, which blends static and dynamic checks in a novel way, in some sense performing better statically than any decidable approximation; (3) a type reconstruction algorithm - reconstruction is decidable even though type checking is not, when suitably redefined to apply to undecidable type systems; (4) a novel use of existential types with dependent types to ensure that the language of logical formulae is closed under type checking (5) a prototype implementation, Sage, of executable refinement types such that all dynamic errors are communicated back to the compiler and are thenceforth static errors.

==> Makefile <==
ALL_TARGETS=main.pdf

TEXINPUTS=
LATEX=TEXINPUTS='$(TEXINPUTS)' latex -interaction=errorstopmode
PDFLATEX=TEXINPUTS='$(TEXINPUTS)' pdflatex 

EXTRAS=includes/brackets.tex \
	main.bbl \
	chapters/intro/main-intro.tex \
	chapters/lambdah/main-lambdah.tex \
	chapters/lambdah/figures/syntax.tex \
	chapters/lambdah/figures/evalrules.tex \
	chapters/lambdah/figures/implication.tex \
	chapters/lambdah/figures/typerules.tex \
	chapters/lambdah/figures/bisimilarity.tex \
	chapters/htc/main-htc.tex \
	chapters/inference/main-inference.tex \
	chapters/compositionality/main-compositionality.tex \
	chapters/sage/main-sage.tex \
	chapters/compositionality/figures/evalrules.tex \
	chapters/compositionality/figures/typerules.tex \
	chapters/relatedwork/main-relatedwork.tex \
	chapters/sage/main-sage.tex

all: $(ALL_TARGETS) 

$(ALL_TARGETS) : $(EXTRAS)

main.ps : $(EXTRAS)

upload : $(UPLOAD_TARGETS)
	scp $(UPLOAD_TARGETS) kenn@169.233.52.218:

slides-6up.ps : slides.ps
	psnup -6 -l -pletter slides.ps > slides-6up.ps

%.ps.gz: %.ps
	gzip -c -f $^ > $@

%.ps: %.dvi
	dvips -t letter -o $@ $<

%.dvi: %.tex
	$(LATEX) $<

%.pdf: %.tex
	$(PDFLATEX) $< $@
	$(PDFLATEX) $< $@

%.aux: %.tex
	$(PDFLATEX) $< $@

%.bbl: %.aux %.bib
	bibtex $(basename $@ .bbl)


==> chapters/htc/figures/bisimilarity.tex <==

\renewcommand{\bisim}{\ensuremath{\sim}}
\renewcommand{\judgesimty}[3]{\ensuremath{#1\vdash #2\,\bisim\,#3}}

% The untyped version.  Just as useful, but uglier and less canonical
\renewcommand{\judgesim}[3]{\ensuremath{#1\vdash #2\,\bisim\,#3}}
% a hackish version used in proofs
\renewcommand{\judgesimmt}[2]{\ensuremath{{#1} \bisim {#2}}}

\renewcommand{\bisimilarityrules}{
  \begin{trules}
    \headtrule{\judgesimty E S T}{
      \underline{Eq}uivalence of types modulo upcasts
      \qquad\qquad\qquad\qquad
      \qquad\qquad\qquad\qquad
    }
  \end{trules}
  \qquad\qquad\qquad
  \[
  \begin{array}[t]{@{}c@{}r@{}}
    \trule{Eq-Arrow}{
      \judgesimty {E} {S_1} {T_1} \qquad
      \judgesimty {E,x:S_1} {S_2} {T_2}
    }{
      \judgesimty E {\lamt x {S_1} {S_2}} {\lamt x {T_1} {T_2}}
    }
  \end{array}
  \qquad
  \begin{array}[t]{@{}c@{}r@{}}
    \trule{Eq-Base}{
      \judgesimt {E,x:B} s t \Bool
    }{
      \judgesimty E {\predty x B s} {\predty x B t}
    }
  \end{array}
  \]

  \
  
  \begin{trules}
    \headtrule{\judgesimt E s t T}{
      Equivalence of terms modulo \underline{up}casts
      \qquad\qquad\qquad\qquad
      \qquad\qquad\qquad\qquad
    }
  \end{trules}
%  \emph{Equivalence and congruence rules:}
  \[
  \begin{array}[t]{@{}c@{}r@{}}
    % I've expanded it just to demonstrate that it is the whole type system!
%    \trule{Up-Refl}{
%      \judge E t T
%	}{
%	  \judgesimt E t t T
%	}
%    \trule{Up-Sym}{
%      \judgesimt E s t T
%    }{
%      \judgesimt E t s T
%    }
    \trule{Up-Equiv}{
      \judgesimt E s t S
      \qquad
      \judgesimty E S T
    }{
      \judgesimt E s t T
    }
    \trule{Up-Trans}{
      \judgesimt E s t T \qquad
      \judgesimt E t u T
    }{
      \judgesimt E s u T
    }
    \trule{Up-Sub}{
      \judgesimt E s t S \qquad
      \judgesub E S T \qquad
    }{
      \judgesimt E s t T
    }
    \trule{Up-Const}{
      ~
    }{
      \judgesimt E c c {ty(c)}
    }
    \trule{Up-Var}{
      (x:T) \in E
    }{
      \judgesimt E x x T
    }
  \end{array}
  \qquad
  \begin{array}[t]{@{}c@{}r@{}}
    \trule{Up-App}{
	  \judgesimt E {s_1} {t_1} {\lamt x {S_1} {S_2}}
      \qquad
	  \judgesimt E {s_2} {t_2} {S_1}
    }{
	  \judgesimt E {s_1~s_2} {t_1~t_2} {\subst x {s_2} {S_1} \, {S_2}}
    }
    \trule{Up-Fun}{
      \judgesimty E {S_1} {T_1}
      \qquad
      \judgesimt {E,x:S_1} s t {S_2}
    }{
	  \judgesimt E {(\lam x {S_1} s)} {(\lam x {T_1} t)} {(\lamt x {S_1} {S_2})}
    }
    \trule{Up-Cast}{
	  \judgesimty E {S_1} {T_1} \qquad
      \judgesimty E {S_2} {T_2}
    }{
	  \judgesimt E {\casttwo {S_1} {S_2}} {\casttwo {T_1} {T_2}} {\arrowt {S_1} {S_2}}
    }
  \end{array}
  \]
  \[
  \begin{array}[t]{@{}c@{}r@{}}
    \trule{Up-Checking}{
      \judgesimt {E,x:B} p q \Bool
      % {\predty{x}{B}{p} = \predty{x}{B}{q}}
      \qquad
      \judgeimp E {\subst x c B\, p} s
      %\subst x c B\, p \red^* s
      \qquad
      \judgeimp E {\subst x c B\, q} t
      %\subst x c B\, q \red^* t
    }{
      \judgesimt E {
        \checkingpred x B p s c
      } { 
        \checkingpred x B q t c
      } {
        \predty x B p
      }
    }
  \end{array}
  \]

  \
  
%  \emph{Extensional equivalence modulo redundant casts (Function casts
%    perform $\eta$-expansion):}
  \[
  \begin{array}[t]{@{}c@{}r@{}}
    \trule{Up-Add}{
      \judgesimt E s t S \qquad
      \judgesub E S T \qquad
	}{
	  \judgesimt E s {\casttwoapp S T t} T
	}
    \trule{Up-Eta}{
      \judgesimt E s t {(\lamt x S T)}
      % \judge E s {\lamt{x}{T}{\_}} ~\clubsuit
      % \qquad
      % \judgesim{E}{t~x}{s}
	}{
	  \judgesimt E s {(\lam x S t~x)} {(\lamt x S T)}
	}
    \trule{Up-AddChecking}{
      \judge E s {\predty x B q}
      \qquad
      \judgesimt E s c {\predty x B q}
      \qquad
      \judgeimp E t {\subst x c B\, q}
      %{\subst x c B}\, q \red^* t
    }{
      \judgesimt E s {\checkingpred x B q t c} {\predty x B q}
    }
  \end{array}
  \]
}



==> chapters/htc/figures/evalrules.tex <==

\newcommand{\htcopsem}{
  \[
  \begin{array}{@{}rclr}
    \headrule{$\tmd \red \e$}{Redex \underline{E}valuation}
    \\
    (\lam x \tyS \e) ~ \tmd      & \red &  {\subst x \tmd S}\, \e & \rel{E-$\beta$}
    \\
    \constant ~ \val             & \red &  \deltaf \constant \val & \rel{E-$\delta$}
    \\
    \\
    \casttwoapp {\lamt x {\tyS_1} {\tyS_2}} {\lamt x {\tyT_1} {\tyT_2}} \f
    &\red& &\rel{\bf E-Cast-F}
    \\
    \multicolumn{4}{l}{
      \qquad\qquad\qquad\funcasttwo x {\tyS_1} {\tyS_2} \f {\tyT_1} {\tyT_2} 
    }
    % funcasttwo x SrcDom SrcRng f DstDom DstRng
    \\
    \\
    \casttwoapp {\predty x B \predq} {\predty x B \predp} \constant
    &\red&
    \checkingpred x B \predp {{\subst x \constant B}\, \predp} \constant
    &\rel{\bf E-Cast-Begin}
    \\
    \checkingpred x B \predq \true \constant
    &\red&
    \constant
    &\rel{\bf E-Cast-End}\\
    \\
    \headrule{\tmctx, \tyctx}{Contexts}
    \\
    \multicolumn{4}{l}{
      \begin{array}{lll}
      \tmctx  & ::= &
      \hole
      ~|~ \app \tmctx \e
      ~|~ \app \e \tmctx
      ~|~ \lam x \tyS \tmctx
      ~|~ \lam x \tyctx \e
      ~|~ \checking \tyT \tmctx \constant
      ~|~ \checking \tyctx \e \constant
      ~|~ \casttwo \tyctx \tyT
      ~|~ \casttwo \tyS \tyctx
      \\
      \tyctx & ::= &
      \lamt x \tyctx \tyT
      ~|~ \lamt x \tyS \tyctx
      ~|~ \predty x B \tmctx
      \end{array}
    }
    \\
  \end{array}
  \]
}


==> chapters/htc/figures/implication.tex <==
\renewcommand{\judgehol}[2]{{#1} \vdash_{CiC} {#2}}

\renewcommand{\implicationaxioms}{ 
\begin{assume}
  We assume that the implication judgement satisfies the following,
  where all environments are assumed to be well-formed, and
  $p,q,r$ are terms of type $\Bool$ in all relevant environments.

  \begin{enumerate}
  \item (Weakening) If $\judgeimp {E,G} p q$ then $\judgeimp {E,x:S,G} p q$.

  \item (Transitivity) 
    If $\judgeimp E p q$ and $\judgeimp E q r$ then $\judgeimp E p r$

  \item (Reflexivity) $\judgeimp E p p$ 
    
  \item (Faithfulness) $\judgeimp E p \true$
  
  \item (Consistency) $\njudgeimp \emptyset \true \false$ 

  \item (Evaluation) If $p \leftrightsquigarrow^* q$ then \judgeimp E p q

  \item (Substitution) If $\judgeimp {E,x:S,F} p q$ and $\judge E t S$ then
    $\judgeimp {E,\theta F} {\theta p} {\theta q}$ where $\theta =
    \subst x t {}$

  \item (Hypothesis) If $ty(c) = \predty x B p$, a singleton type
    by Assumption \ref{assume:consts},
    and $\judgeimp E \true {\subst x c {ty(c)}\, p}$
    then $\judgeimp {E,x:B} {x = c} {p}$

  \item (Narrowing) If $\judgeimp {E,x:T,F} p q$ and $\judgesub E S T$
    then $\judgeimp {E,x:S,F} p q$

  \end{enumerate}
  \end{assume}
}

\renewcommand{\implicationprojection}{
  \begin{trules}
    \headtrule {\judgeimp E p q} {\underline{Imp}lication}
    \trule{Imp}{
      \forall \sigma.\, 
      (E\models \sigma 
      \mbox{ and } 
      \sigma(p) \rightarrow^* \true)
      \mbox{ implies } 
      sigma(q) \rightarrow^* \true
    }{
      \judgeimp E p q
    }
    \headtrule{$E\models\sigma$} {\underline{C}losing \underline{S}ubstitutions}
    \trule{CS}{
      \forall i.~~ \sigma_i = \subst {x_i} {t_i} {T_i}
      $ where $ t_i \in \meaningf{T_i}
      $ and $ fv(t_i) \subseteq \{x_j ~|~ j < i\}
    }{
      x_1:T_1, \cdots, x_n:T_n ~\models~ \sigma_1 \circ \cdots \circ \sigma_n
    }
  \end{trules}
  
  And $\meaningf{T} = \{ \castapp T t ~|~ t \in Term \}$
}

\renewcommand{\STLC}[1]{\ensuremath{\lfloor {#1} \rfloor}}
\renewcommand{\Base}[1]{\ensuremath{\lfloor {#1} \rfloor}}
\renewcommand{\limit}[2]{\ensuremath{{#1}\!\!\downharpoonright_{#2}}}

\renewcommand{\implicationquotient}{
  \

  \qquad\qquad\qquad % \centering \begin{center} etc do nothing wtf
  \begin{tabular}{cc}
    \(
    \begin{array}[t]{rcl}
      \Base {\predty x B t} & = & B \\
      \Base {\lamt x S T} & = & \arrowt {\Base S} {\Base T}\\
    \end{array}
    \)
    &
    \(
    \begin{array}[t]{rcl}
      \Base c & = & c\\
      \Base x & = & x\\
      \Base {\lam x S t} & = & \lam x {\Base S} {\Base t} \\
      \Base {t_1~t_2} & = & \Base {t_1} ~ \Base {t_2} \\
      \Base {\casttwo S T} & = & \casttwo S T \\
      \Base {\checking T t c} & = & \checking {\Base T} {\Base t} c\\
    \end{array}
    \)
  \end{tabular}

  \

  \begin{eqnarray*}
    \meaningf {\predty x B s}
    & = & 
    \{ t ~|~ \judgeS {} {\Base t} B
    ~\wedge~ 
    (t \lred^* c \mbox{ implies } \subst x c B\, s \lred^* \true) \} 
    \\
    \meaningf {\lamt x S T} 
    & = &
    \{
    t ~|~ \judgeS {} {\Base t} {\arrowt {\Base S} {\Base T}}
    ~\wedge~ \forall s \in \meaningf{S},~ 
    t~s \in \meaningf{\subst x s S\, T}
    \}
  \end{eqnarray*}
  
  \ 

  \begin{trules}
    \trule{Subst}{
      \forall x \in dom(E),~
      \sigma(x) 
      \in \meaningf{\sigma(E(x))}
    }{
      \judge {} \sigma E
    }
    \\
    \trule{Imp}{
      \forall \sigma. \mbox{ if } \judge {} \sigma E 
      \mbox{ and } \sigma(p) \lred^* \true
      \mbox{ then } \sigma(q) \lred^* \true
    }{
      \judgeimp E p q
    }
  \end{trules}
}

\renewcommand{\implicationhol}{
  \begin{eqnarray*}
    \Base ~ & :: & LambdaHType \rightarrow STLCType \\
    \Base {\predty x B p} & = & \bar B \\
    \Base {\lamt x S T} & = & \Base S \rightarrow \Base T \\
    \\
    \STLC {~} & :: & LambdaHTerm \rightarrow STLCTerm \\
    \STLC x & = & \bar x \\
    \STLC c & = & \bar c \\
    \STLC {\lam x T t} & = & \lam {\bar x} {Base(T)} {STLC(t)} \\
    \STLC {s~t} & = & \STLC s ~ \STLC t \\
    \STLC {\casttwo {\predty x B p} {\predty x B q}}
    & = & \lam {\bar x} B {\t{if} ~  \STLC q ~ \t{then} ~ \bar x ~ \t{else} ~ 
      \t{barf}} \\
    \STLC {\casttwo {\lamt x S T} {\lamt x U V}} 
    & = &
    \lam {\bar f} {\Base {\lamt x S T}} {}
    \lam {\bar x} {\Base U} {} \\
    && \qquad \STLC {\casttwo T V}~(\bar f~(\STLC {\casttwo U S}~\bar x))
    \\
    \\
    \meaningf {~} & :: & LambdaHType \rightarrow \mathcal{P}(LambdaHTerm) \\
    \meaningf {\predty x B p} 
    & = & \{ t ~|~ \judgeS {} {\STLC t} \bar B \mbox{ and }
    \subst x t B\, p \lred^* \true \} \\
    \meaningf {\lamt x S T} & = &
    \{
    t ~|~ \judgeS {} {\STLC t} \Base{\lamt x S T} 
    \mbox{ and } \forall t', t' \in \meaningf{S} 
    \mbox{ implies } t~t' \in \meaningf{\subst x t' {}\, T}
    \}
  \end{eqnarray*}
  \ \\
  \begin{trules}
    \trule{Subst}{
      \forall x \in dom(E), 
      {\limit \sigma x}(x) 
      \in \meaningf{{\limit \sigma x}(E(x))}
    }{
      \judge {} \sigma E
    }
    \\
    \trule{Imp}{
      \forall \sigma. \mbox{ if } \judge {} \sigma E 
      \mbox{ and } \sigma(p) \lred^* \true
      \mbox{ then } \sigma(q) \lred^* \true
    }{
      \judgeimp E p q
    }
  \end{trules}
%  
%  where
%
%    \\
%    Translate & :: & ImpJudgement \rightarrow CicJudgement \\
%    Translate(\judgeimp E p q) & = & 
%    \judgehol {Meta(E), Pre(E)} 
%    {STLC(p) \lred^* \true 
%%      \rightarrow STLC(q) \lred^* \true}
%    \\
%%    && \mbox{ where } p' = \subst {x_{STLC}} {\bar x} {} STLC(p) \\
%    && \mbox{ and similarly for } q' \mbox{ for all } x\\
%    \\
%    Meta & :: & LambdaHEnv \rightarrow CicEnv \\
%    Meta(\emptyset) & = & \bar{\emptyset} \\
%    Meta(x:T) & = & \bar{x} : STLCTerm \\
%    \\
%    Pre & :: & LambdaHEnv \rightarrow CicEnv \\
%    Pre(\emptyset) & = & \true_{CiC} \\
%    Pre(E,x:T) 
%    & = & Pre(E),
%    (\judgeS {Base(E)} {\bar{x}} {Base(T)})
%    \wedge Predicate(T, \bar{x}) \\
%    \\
%    Predicate & :: & (CiCEnv,LambdaHType, STLCTerm) \rightarrow CicPred \\
%    Predicate(E, \predty x B p, y) 
%    & = & \subst {x_{STLC}} y B\, STLC(p) \lred^* \true \\
%    Predicate(E, (\lamt x S T), f) & = & 
%    \forall x:STLCTerm.\judgeS {} {Base(S) \wedge Predicate(S,x) \rightarrow (Predicate(T,f~x)) \\
%    \\
%  \end{eqnarray*}
}



==> chapters/htc/figures/syntax.tex <==

% Just the casts
\newcommand{\htcsyntax}{
  \[
  \begin{array}{llr}
    \mydefhead {\e,\tmd,\tmf,\g,\predq,\predp ::=\qquad\qquad\qquad\qquad\qquad} {Terms:} 
    \mydefcase \constant                                                         {constant} 
    \mydefcase x                                                                 {variable} 
    \mydefcase {\lam x \tyS \e}                                                  {abstraction} 
    \mydefcase {\tmf ~ \e}                                                       {application} 
    \mydefcase {\casttwo \tyS \tyT}                                              {\bf \emph{type cast}} 
    \mydefcase {\checking {\predty x B \predp} \predq \constant}                 {\bf \emph{cast in progress}}
    \\
    \mydefhead {\val ::=\qquad\qquad\qquad\qquad\qquad} {Values: ($\subset$ Terms)}
    \mydefcase \constant                                {constant} 
    \mydefcase {\lam x \tyS \e}                         {abstraction} 
    \mydefcase {\casttwo \tyS \tyT}                     {\bf \emph{type cast}} 
    \\
    \mydefhead {\tyS,\tyT,\tyU::=}    {Types:} 
    \mydefcase {\lamt x \tyS \tyT}    {dependent function type}
    \mydefcase {\predty x B \predp}   {refined basic type} 
  \end{array}
  \]
}



==> chapters/htc/figures/typerules.tex <==

\newcommand{\htctyperules}{
  \headtrule{$\judge{E}{\e}{T}$}{Additional \underline{T}ype rules}
  \begin{trules}
    \trule{T-Cast}{
      \judgeT \env \tyS \qquad
      \judgeT \env \tyT \qquad
      \Base \tyS = \Base \tyT
    }{
      \judge \env {\casttwo \tyS \tyT} {\arrowt \tyS \tyT}
    }
    
    \trule{T-Checking}{
      \judgeT \env {\predty x B \predp}
      \and
      \judge \env \constant B 
      \and
      \judge \env \predq \Bool
      \and
      \judgeimp \env \predq {\subst x \constant B\, \predp}
    }{
      \judge \env {\checkingpred x B \predp \predq \constant} {\predty x B \predp}
    }
  \end{trules}
}


==> chapters/inference/brackets.tex <==
% ---------------------------------------------------------------------	%
% Horizontal brackets.							%
% ---------------------------------------------------------------------	%

\newcommand{\hbra}{
\hbox to \textwidth{\vrule width0.3mm height 1.8mm depth-0.3mm
                    \leaders\hrule height1.8mm depth-1.5mm\hfill
                    \vrule width0.3mm height 1.8mm depth-0.3mm}}
\newcommand{\hket}{
\hbox to \textwidth{\vrule width0.3mm height1.5mm
                    \leaders\hrule height0.3mm\hfill
                    \vrule width0.3mm height1.5mm}}


\renewcommand{\hbra}{
\hbox to \columnwidth{\vrule width0.3mm height 1.8mm depth-0.3mm
                    \leaders\hrule height1.8mm depth-1.5mm\hfill
                    \vrule width0.3mm height 1.8mm depth-0.3mm}}
\renewcommand{\hket}{
\hbox to \columnwidth{\vrule width0.3mm height1.5mm
                    \leaders\hrule height0.3mm\hfill
                    \vrule width0.3mm height1.5mm}}


%\newcounter{figure}


\newenvironment{display}[1]{
  \refstepcounter{figure}
 % \begin{tabbing}
 % \hspace{1.5em} \= \hspace{.40\linewidth - 2em} \= \hspace{2em} \= \kill
%  \medskip
\noindent
  \textbf{Figure~\thefigure:  #1}\\
  \hbra\\[-.8ex]
  \nopagebreak
  %\small
 }{ 
 \\[-2ex]
 \nopagebreak
  \hket
  \nopagebreak
% \medskip
 % \end{tabbing}
 }


\newcommand{\htbra}{
\hbox to \textwidth{\vrule width0.3mm height 1.8mm depth-0.3mm
                    \leaders\hrule height1.8mm depth-1.5mm\hfill
                    \vrule width0.3mm height 1.8mm depth-0.3mm}}
\newcommand{\htket}{
\hbox to \textwidth{\vrule width0.3mm height1.5mm
                    \leaders\hrule height0.3mm\hfill
                    \vrule width0.3mm height1.5mm}}


\newenvironment{displayfigure}[2][t!]{
  \begin{figure}[#1]
  \refstepcounter{figure}
  \medskip
  \textbf{Figure~\thefigure:  #2}\\
  \hbra\\[-.8ex]
 }{ 
  \\[-.8ex]
  \hket
  \medskip
  \end{figure}
 }

\newenvironment{displayfigure*}[2][th!]{
  \begin{figure*}[#1]
  \refstepcounter{figure}
  \medskip
  \textbf{Figure~\thefigure:  #1}\\
  \htbra\\[-.8ex]
 }{ 
  \\[-.8ex]
  \htket
  \medskip
  \end{figure*}
 }

\newenvironment{displayname}[1]{
  \refstepcounter{figure}
  \begin{tabbing}
  \hspace{1.5em} \= \hspace{.40\linewidth - 2em} \= \hspace{2em} \= \kill
  \textbf{Figure~\thefigure: #1}\\[-.8ex]
  \hbra\\[-.8ex]
  \nopagebreak
 }{
  \\[-.8ex]\hket

  \end{tabbing}
 }

%%%%%%%% typesetting type rules %%%%%%%%%%%%%
\newenvironment{trules}
{\[\begin{array}{@{}c@{}r@{}}}
{\end{array}\]}
\newcommand{\headtrule}[2]{
	\multicolumn{2}{@{}l@{}}{\mbox{#2}} \hfil \fbox{#1}\\
	\multicolumn{2}{@{}l@{}}{\hskip3.25in}\\
}

\newcommand{\trule}[3]{
\frac 
	{\strut\begin{array}{@{}c@{}} #2 \end{array}} 
	{\strut\begin{array}{@{}c@{}} #3 \end{array}}
&\rel{#1} \\~\\
}

\newcommand{\trulenoname}[2]{
\frac 
	{\strut\begin{array}{@{}c@{}} #1 \end{array}} 
	{\strut\begin{array}{@{}c@{}} #2 \end{array}}
}

\newcommand{\rtrule}[3]{  % restatement in proof
Suppose $#3$ via the rule:
\[
\frac
      {\strut\begin{array}{@{}c@{}} #2 \end{array}}
     {\strut\begin{array}{@{}c@{}} #3 \end{array}}
\qquad\rel{#1}
\]
}
\newcommand{\trulespc}[4]{
\frac
      {\strut\begin{array}{@{}c@{}} #2 \end{array}}
      {\strut\begin{array}{@{}c@{}} #3 \end{array}}
}

\newcommand{\nrln}[3]{
\mbox{
$\begin{array}{l}
\rel{#1} \\
\quad\frac 
	{\strut\begin{array}{c} #2 \end{array}} 
	{\strut\begin{array}{c} #3 \end{array}}
\end{array}
$}}

\newcommand{\rel}[1]{\raisebox{0ex}[0ex][0ex]{\small [\textsc{#1}}]}
%\newcommand{\mydefhead}[2]{\multicolumn{2}{l}{{#1}}&\mbox{\emph{#2}}\\}
\newcommand{\mydefhead}[2]{{#1}\\}
%\newcommand{\mydefcase}[2]{\qquad& #1 &\mbox{#2}\\}
\newcommand{\mydefcase}[2]{\qquad&{#1}\\}
\newcommand{\headrule}[2]{\multicolumn{3}{@{}l}{\mbox{#2}} & \fbox{#1}\\}


\newcommand{\proofcomplete}{\ensuremath{\square}}
\newenvironment{myproof}%
  {%\begin{quote}
    %\item[]
%   \begin{quote}
\emph{Proof:}
%     \normalsize{\sc Proof:}\hspace*{0mm}
}
  {\proofcomplete\newline
%\end{quote}%
%\smallskip
   }


==> chapters/inference/figures/constraintgen.tex <==
\newcommand{\constraintgenrules}{
  \headtrule{
    $\judgeC \env \e T C$
  }{
    \underline{C}onstraint \underline{G}eneration rules
  }
  \begin{trules}
    \trule{CG-Var}{ (x:T)\in \env }{ \judgeC{\env}{x}{T}{\emptyset} }

    \trule{CG-Const}{ \\ }{ \judgeC{\env}{\constant}{\fun{ty}(\constant)}{\emptyset} }
    
    %\trule{CG-PH}{ \\ }{ \judgeC{\env}{\theta \dapp \ph}{\Bool}{\emptyset} }
    
    \trule{CG-Fun}{
      \judgeTC{\env}{S}{C_1} \qquad
      \judgeC{\env,x:S}{\e}{T}{C_2}
    }{
      \judgeC{\env}{(\lam{x}{S}{\e})}{(\lamt{x}{S}{T})}{C_1 \cup C_2}
    }
    
    \trule{CG-App}{
      \judgeC{\env}{\f}{T}{C_1} \\ 
      \judgeC{\env}{\e}{S}{C_2} \\
      \alpha \textnormal{ fresh } \\
    }{
      \judgeC{\env}{
        \f~\e
      }{
        \substT{x}{\e}{S} \dapp \alpha
        ~
      }{
        ~
        C_1 \cup C_2 \cup
        \{ 
        \judgeT {\env,x\!:\!S} \tyvar,~
        \judgesub \env T {(\lamt x S \tyvar})
        \}
      }
    }
  \end{trules}
}
 
\newcommand{\typeconstraintgenrules}{ 
  \headtrule{
    $\judgeTC{\env}{T}{C}$
  }{
    \underline{W}ell-formed \underline{T}ype \underline{C}onstraint Generation
  }
  \begin{trules}
  \trule{WTC-Arrow}{ 
      \judgeTC{\env}{S}{C_1} \qquad \judgeTC{\env,x:S}{T}{C_2} 
    }{
      \judgeTC \env {\lamt x S T ~} {~ C_1 \cup C_2}
    }

    \trule{WTC-Base}{
      %       x\not\in\fun{dom}(\env) \qquad
      \judgeC{\env,x:B}{\e}{\Bool}{C}
    }{
      \judgeTC{\env}{\predty{x}{B}{\e}}{C}
    }

    \trule{WTC-Var}{ \\
    }{
      \judgeTC{\env}{\alpha}{\{\judgeT \env \tyvar\}}
    }
  \end{trules}
}


==> chapters/inference/figures/syntax.tex <==

\newcommand{\syntaxtostaterecon}{
  \[
  \begin{array}{llr}
    \mydefhead{\e,\tmd,\tmf,\g,\predq,\predp ::=\qquad\qquad\qquad\qquad\qquad} {Terms:} 
    \mydefcase \constant                                                        {constant} 
    \mydefcase x                                                                {variable} 
    \mydefcase {\lam x \tyS \e}                                                 {abstraction} 
    \mydefcase {\tmf~\e}                                                        {application} 
    \\
    \mydefhead {\val ::=\qquad\qquad\qquad\qquad\qquad} {Values: ($\subset$ Terms)}
    \mydefcase \constant                                {constant} 
    \mydefcase {\lam x \tyS \e}                         {abstraction} 
    \\
    \mydefhead {R,\tyS,\tyT,\tyU::=}    {Types:} 
    \mydefcase {\lamt x \tyS \tyT}      {dependent function type}
    \mydefcase {\predty x B \predp}     {refined basic type} 
    \mydefcase \tyvar                   {\bf \emph{type variable}} 
  \end{array}
  \]
}

\newcommand{\constraintgensyntax}{
  \[
  \begin{array}{llr}
    \mydefhead {\e,\tmd,\tmf,\g,\predq,\predp ::=\qquad\qquad\qquad\qquad\qquad} {Terms:} 
    \mydefcase \constant                                                         {constant} 
    \mydefcase x                                                                 {variable} 
    \mydefcase{\lam x \tyS \e}                                                   {abstraction} 
    \mydefcase {\tmf ~ \e}                                                       {application} 
    \\
    \mydefhead {\val ::=\qquad\qquad\qquad\qquad\qquad} {Values: ($\subset$ Terms)}
    \mydefcase \constant                                {constant} 
    \mydefcase {\lam x \tyS \e}                         {abstraction} 
    \\
    \mydefhead {R,\tyS,\tyT,\tyU::=}    {Types:} 
    \mydefcase {\lamt x \tyS \tyT}      {dependent function type}
    \mydefcase {\predty x B \predp}     {refined basic type} 
    \mydefcase {\dsub\dapp\tyvar}       {\bf \emph{type variable with substitution}} 
    \\
    \mydefhead {\dsub ::=}                      {Delayed substitution}
    \mydefcase \emptysubst                      {empty substitution}
    \mydefcase {{\substT x \e T} \circ \dsub}   {substitution extension}
    \\
    \mydefhead {\judgesub \env S T}    {Subtyping constraint}
    \\
    \mydefhead {\judgeT \env T}        {Type well-formedness constraint}
  \end{array}
  \]
}

\newcommand{\shapereconsyntax}{
  \[
  \begin{array}{llr}
    \mydefhead{\predp,\predq ::=\qquad\qquad\qquad\qquad\qquad} {Predicates:} 
    \mydefcase {\dsub\dapp\ph}     {\bf \emph{placeholder with substitution}} 
    \mydefcase \e                  {term}
    \\
    \mydefhead{\e,\tmd,\tmf,\g ::=\qquad\qquad\qquad\qquad\qquad} {Terms:} 
    \mydefcase{\constant                              }{constant} 
    \mydefcase x                                                                {variable} 
    \mydefcase{\lam{x}{\tyS}{\e} 		              }{abstraction} 
    \mydefcase {\tmf~\e}                                                        {application} 
    \\
    \mydefhead{\val ::=\qquad\qquad\qquad\qquad\qquad}{Values: ($\subset$ Terms)}
    \mydefcase{\constant                              }{constant} 
    \mydefcase{\lam{x}{\tyS}{\e} 		              }{abstraction} 
    \\
    \mydefhead {R,\tyS,\tyT,\tyU::=}    {Types:} 
    \mydefcase {\lamt x \tyS \tyT}    {dependent function type}
    \mydefcase {\predty x B \predp}   {refined basic type} 
    \\
    \mydefhead {\dsub ::=}                      {Delayed substitution}
    \mydefcase \emptysubst                      {empty substitution}
    \mydefcase {{\substT x \e T} \circ \dsub}   {substitution extension}
    \\
    \mydefhead {\judgeimp \env \predp \predq}    {Implication constraint}
    \\
    \mydefhead {\judge \env \predp \Bool}        {Refinement well-typedness constraint}
  \end{array}
  \]
}

\newcommand{\finalinferencesyntax}{
  \[
  \begin{array}{llr}
    \mydefhead{\e,\tmd,\tmf,\g,\predq,\predp ::=\qquad\qquad\qquad\qquad\qquad} {Terms:} 
    \mydefcase{\constant                              }{constant} 
    \mydefcase{\lam{x}{\tyS}{\e} 		              }{abstraction} 
    \mydefcase x                                                                {variable} 
    \mydefcase {\tmf~\e}                                                        {application} 
    \mydefcase {\existstm x T \predp}                                           {\bf \emph{existential quantification}}
    \mydefcase {\e \vee \e}                                                     {\bf \emph{parallel disjunction}}
    \mydefcase {\e \wedge \e}                                                   {\bf \emph{parallel conjunction}}
    \\
    \mydefhead{\val ::=\qquad\qquad\qquad\qquad\qquad}{Values: ($\subset$ Terms)}
    \mydefcase{\constant                              }{constant} 
    \mydefcase{\lam{x}{\tyS}{\e} 		              }{abstraction} 
    \\
    \mydefhead {R,\tyS,\tyT,\tyU::=}    {Types:} 
    \mydefcase {\lamt x \tyS \tyT}    {dependent function type}
    \mydefcase {\predty x B \predp}   {refined basic type} 
  \end{array}
  \]
}



==> chapters/lambdah/figures/bisimilarity.tex <==

% The untyped version.  Just as useful, but uglier and less canonical
\newcommand{\judgesim}[3]{\ensuremath{#1\vdash #2\,\bisim\,#3}}
% a hackish version used in proofs
\newcommand{\judgesimmt}[2]{\ensuremath{{#1} \bisim {#2}}}

\newcommand{\tysimilarity}{
  \headtrule{$\judgesimty E S T$}{
    \underline{Eq}uivalence of types modulo upcasts
  }
  \begin{trules}
    \trule{Eq-Arrow}{
      \judgesimty {E} {S_1} {T_1} \qquad
      \judgesimty {E,x:S_1} {S_2} {T_2}
    }{
      \judgesimty E {\lamt x {S_1} {S_2}} {\lamt x {T_1} {T_2}}
    }

    \trule{Eq-Base}{
      \judgesimt {E,x:B} s t \Bool
    }{
      \judgesimty E {\predty x B s} {\predty x B t}
    }
  \end{trules}
}

% \emph{Equivalence and congruence rules:}
\newcommand{\bisimilarityrules}{
  \headtrule{$\judgesimt E s t T$}{
    Equivalence of terms modulo \underline{up}casts
  }
  \begin{trules}
    % I've expanded it just to demonstrate that it is the whole type system!
%    \trule{Up-Refl}{
%      \judge E t T
%	}{
%	  \judgesimt E t t T
%	}
%    \trule{Up-Sym}{
%      \judgesimt E s t T
%    }{
%      \judgesimt E t s T
%    }
    \trule{Up-Equiv}{
      \judgesimt E s t S
      \qquad
      \judgesimty E S T
    }{
      \judgesimt E s t T
    }

    \trule{Up-Trans}{
      \judgesimt E s t T \qquad
      \judgesimt E t u T
    }{
      \judgesimt E s u T
    }

    \trule{Up-Sub}{
      \judgesimt E s t S \qquad
      \judgesub E S T \qquad
    }{
      \judgesimt E s t T
    }

    \trule{Up-Const}{
      ~
    }{
      \judgesimt E c c {ty(c)}
    }

    \trule{Up-Var}{
      (x:T) \in E
    }{
      \judgesimt E x x T
    }
    
    \trule{Up-App}{
	  \judgesimt E {s_1} {t_1} {\lamt x {S_1} {S_2}}
      \qquad
	  \judgesimt E {s_2} {t_2} {S_1}
    }{
	  \judgesimt E {s_1~s_2} {t_1~t_2} {\subst x {s_2} {S_1} \, {S_2}}
    }

    \trule{Up-Fun}{
      \judgesimty E {S_1} {T_1}
      \qquad
      \judgesimt {E,x:S_1} s t {S_2}
    }{
	  \judgesimt E {(\lam x {S_1} s)} {(\lam x {T_1} t)} {(\lamt x {S_1} {S_2})}
    }

    \trule{Up-Cast}{
	  \judgesimty E {S_1} {T_1} \qquad
      \judgesimty E {S_2} {T_2}
    }{
	  \judgesimt E {\casttwo {S_1} {S_2}} {\casttwo {T_1} {T_2}} {\arrowt {S_1} {S_2}}
    }

    \trule{Up-Checking}{
      \judgesimt {E,x:B} p q \Bool
      % {\predty{x}{B}{p} = \predty{x}{B}{q}}
      \qquad
      \judgeimp E {\subst x c B\, p} s
      %\subst x c B\, p \red^* s
      \qquad
      \judgeimp E {\subst x c B\, q} t
      %\subst x c B\, q \red^* t
    }{
      \judgesimt E {
        \checkingpred x B p s c
      } { 
        \checkingpred x B q t c
      } {
        \predty x B p
      }
    }
  \end{trules}

%  \emph{Extensional equivalence modulo redundant casts (Function casts
%    perform $\eta$-expansion):}
  \begin{trules}
    \trule{Up-Add}{
      \judgesimt E s t S \qquad
      \judgesub E S T \qquad
	}{
	  \judgesimt E s {\casttwoapp S T t} T
	}

    \trule{Up-Eta}{
      \judgesimt E s t {(\lamt x S T)}
      % \judge E s {\lamt{x}{T}{\_}} ~\clubsuit
      % \qquad
      % \judgesim{E}{t~x}{s}
	}{
	  \judgesimt E s {(\lam x S t~x)} {(\lamt x S T)}
	}

    \trule{Up-AddChecking}{
      \judge E s {\predty x B q}
      \qquad
      \judgesimt E s c {\predty x B q}
      \qquad
      \judgeimp E t {\subst x c B\, q}
      %{\subst x c B}\, q \red^* t
    }{
      \judgesimt E s {\checkingpred x B q t c} {\predty x B q}
    }
  \end{trules}
}


==> chapters/lambdah/figures/evalrules.tex <==

% Operational semantics of lambda-H without casts
\newcommand{\basicopsem}{
  \[
  \begin{array}{@{}rclr}
    \headrule{$\tmd \red \e$}{Redex \underline{E}valuation}
    \\
    (\lam x \tyS \tmd) ~ \e      & \red &  {\subst x \e S}\, \tmd & \rel{E-$\beta$}
    \\
    \constant ~ \val             & \red &  \deltaf \constant \val & \rel{E-$\delta$}
    \\
    \\
    \\
    \headrule{$\tmd \lred \e$, $S \lred T$}{Contextual \underline{E}valuation}
    \\
    \qquad\qquad\qquad	\tmctx[\tmd] & \lred & \tmctx[\e] \quad \mbox{if $\tmd \red \e$}
    &\rel{E-Compat} \\
    \qquad\qquad\qquad	\tyctx[\tmd] & \lred & \tyctx[\e] \quad \mbox{if $\tmd \red \e$}
    &\rel{E-TyCompat} \\
    \\
    \headrule{\tmctx, \tyctx}{Contexts}
    \\
    \multicolumn{4}{l}{
      \begin{array}{lll}
      \tmctx  & ::= &
      \hole
      ~|~ \app \tmctx \e
      ~|~ \app \e \tmctx
      ~|~ \lam x \tyS \tmctx
      ~|~ \lam x \tyctx \e
      \\
      \tyctx & ::= &
      \lamt x \tyctx \tyT
      ~|~ \lamt x \tyS \tyctx
      ~|~ \predty x B \tmctx
    \end{array}
    }
    \\
  \end{array}
  \]
}




==> chapters/lambdah/figures/implication.tex <==
\newcommand{\judgehol}[2]{{#1} \vdash_{CiC} {#2}}
\newcommand{\isvalid}{\ensuremath{\lred^* \true}}

\newcommand{\implicationaxioms}{ 
\begin{assume}
  We assume that the implication judgement satisfies the following,
  where all environments are assumed to be well-formed, and
  $p,q,r$ are terms of type $\Bool$ in all relevant environments.

  \begin{enumerate}
  \item (Weakening) If $\judgeimp {E,G} p q$ then $\judgeimp {E,x:S,G} p q$.

  \item (Transitivity) 
    If $\judgeimp E p q$ and $\judgeimp E q r$ then $\judgeimp E p r$

  \item (Reflexivity) $\judgeimp E p p$ 
    
  \item (Faithfulness) $\judgeimp E p \true$
  
  \item (Consistency) $\njudgeimp \emptyset \true \false$ 

  \item (Evaluation) If $p \leftrightsquigarrow^* q$ then \judgeimp E p q

  \item (Substitution) If $\judgeimp {E,x:S,F} p q$ and $\judge E t S$ then
    $\judgeimp {E,\theta F} {\theta p} {\theta q}$ where $\theta =
    \subst x t {}$

  \item (Hypothesis) If $ty(c) = \predty x B p$, a singleton type
    by Assumption \ref{assume:consts},
    and $\judgeimp E \true {\subst x c {ty(c)}\, p}$
    then $\judgeimp {E,x:B} {x = c} {p}$

  \item (Narrowing) If $\judgeimp {E,x:T,F} p q$ and $\judgesub E S T$
    then $\judgeimp {E,x:S,F} p q$

  \end{enumerate}
  \end{assume}
}

\newcommand{\implicationprojection}{
  \begin{trules}
    \headtrule {\judgeimp E p q} {\underline{Imp}lication}
    \trule{Imp}{
      \forall \sigma.\, 
      (E\models \sigma 
      \mbox{ and } 
      \sigma(p) \rightarrow^* \true)
      \mbox{ implies } 
      sigma(q) \rightarrow^* \true
    }{
      \judgeimp E p q
    }
    \headtrule{$E\models\sigma$} {\underline{C}losing \underline{S}ubstitutions}
    \trule{CS}{
      \forall i.~~ \sigma_i = \subst {x_i} {t_i} {T_i}
      $ where $ t_i \in \meaningf{T_i}
      $ and $ fv(t_i) \subseteq \{x_j ~|~ j < i\}
    }{
      x_1:T_1, \cdots, x_n:T_n ~\models~ \sigma_1 \circ \cdots \circ \sigma_n
    }
  \end{trules}
  
  And $\meaningf{T} = \{ \castapp T t ~|~ t \in Term \}$
}

\newcommand{\STLC}[1]{\ensuremath{\lfloor {#1} \rfloor}}
\newcommand{\limit}[2]{\ensuremath{{#1}\!\!\downharpoonright_{#2}}}

\newcommand{\quotientmodel}{
  \begin{eqnarray*}
    \meaningf {\predty x B p}
    & = & 
    \{ t ~|~ \judgeS {} {\Base t} B
    ~\wedge~ 
    (\subst x t B\, p \isvalid \vee t\!\uparrow)\} 
    \\
    \meaningf {\lamt x S T} 
    & = &
    \{
    t ~|~ \judgeS {} {\Base t} {\Base {\lamt x S T}}
    ~\wedge~ \forall s \in \meaningf{S},~ 
    t~s \in \meaningf{\subst x s S\, T}
    \}
  \end{eqnarray*}
}

\newcommand{\closingsubstrule}{
  \begin{trules}
    \trule{Subst}{
      \judgeE E
      \qquad
      \forall x \in dom(E),~
      \sigma(x) 
      \in \meaningf{\sigma(E(x))}
    }{
      \judge {} \sigma E
    }
  \end{trules}
}

\newcommand{\judgequotient}{
  \begin{trules}
    \trule{}{
      \forall \sigma. \mbox{ if } \judge {} \sigma E
      \mbox{ then } \sigma(t) \in \meaningf {\sigma T}
    }{
      \judgeIn E t T
    }
  \end{trules}
}

\newcommand{\implicationquotient}{
  \begin{trules}
    \trule{Imp}{
      \forall \sigma. \mbox{ if } \judge {} \sigma E 
      \mbox{ and } \sigma(p) \isvalid
      \mbox{ then } \sigma(q) \isvalid
    }{
      \judgeimp E p q
    }
  \end{trules}
}

\newcommand{\implicationhol}{
  \begin{eqnarray*}
    \Base ~ & :: & LambdaHType \rightarrow STLCType \\
    \Base {\predty x B p} & = & \bar B \\
    \Base {\lamt x S T} & = & \Base S \rightarrow \Base T \\
    \\
    \STLC {~} & :: & LambdaHTerm \rightarrow STLCTerm \\
    \STLC x & = & \bar x \\
    \STLC c & = & \bar c \\
    \STLC {\lam x T t} & = & \lam {\bar x} {Base(T)} {STLC(t)} \\
    \STLC {s~t} & = & \STLC s ~ \STLC t \\
    \STLC {\casttwo {\predty x B p} {\predty x B q}}
    & = & \lam {\bar x} B {\t{if} ~  \STLC q ~ \t{then} ~ \bar x ~ \t{else} ~ 
      \t{barf}} \\
    \STLC {\casttwo {\lamt x S T} {\lamt x U V}} 
    & = &
    \lam {\bar f} {\Base {\lamt x S T}} {}
    \lam {\bar x} {\Base U} {} \\
    && \qquad \STLC {\casttwo T V}~(\bar f~(\STLC {\casttwo U S}~\bar x))
    \\
    \\
    \meaningf {~} & :: & LambdaHType \rightarrow \mathcal{P}(LambdaHTerm) \\
    \meaningf {\predty x B p} 
    & = & \{ t ~|~ \judgeS {} {\STLC t} \bar B \mbox{ and }
    \subst x t B\, p \lred^* \true \} \\
    \meaningf {\lamt x S T} & = &
    \{
    t ~|~ \judgeS {} {\STLC t} \Base{\lamt x S T} 
    \mbox{ and } \forall t', t' \in \meaningf{S} 
    \mbox{ implies } t~t' \in \meaningf{\subst x t' {}\, T}
    \}
  \end{eqnarray*}
  \ \\
  \begin{trules}
    \trule{Subst}{
      \forall x \in dom(E), 
      {\limit \sigma x}(x) 
      \in \meaningf{{\limit \sigma x}(E(x))}
    }{
      \judge {} \sigma E
    }
    \\
    \trule{Imp}{
      \forall \sigma. \mbox{ if } \judge {} \sigma E 
      \mbox{ and } \sigma(p) \lred^* \true
      \mbox{ then } \sigma(q) \lred^* \true
    }{
      \judgeimp E p q
    }
  \end{trules}
%  
%  where
%
%    \\
%    Translate & :: & ImpJudgement \rightarrow CicJudgement \\
%    Translate(\judgeimp E p q) & = & 
%    \judgehol {Meta(E), Pre(E)} 
%    {STLC(p) \lred^* \true 
%%      \rightarrow STLC(q) \lred^* \true}
%    \\
%%    && \mbox{ where } p' = \subst {x_{STLC}} {\bar x} {} STLC(p) \\
%    && \mbox{ and similarly for } q' \mbox{ for all } x\\
%    \\
%    Meta & :: & LambdaHEnv \rightarrow CicEnv \\
%    Meta(\emptyset) & = & \bar{\emptyset} \\
%    Meta(x:T) & = & \bar{x} : STLCTerm \\
%    \\
%    Pre & :: & LambdaHEnv \rightarrow CicEnv \\
%    Pre(\emptyset) & = & \true_{CiC} \\
%    Pre(E,x:T) 
%    & = & Pre(E),
%    (\judgeS {Base(E)} {\bar{x}} {Base(T)})
%    \wedge Predicate(T, \bar{x}) \\
%    \\
%    Predicate & :: & (CiCEnv,LambdaHType, STLCTerm) \rightarrow CicPred \\
%    Predicate(E, \predty x B p, y) 
%    & = & \subst {x_{STLC}} y B\, STLC(p) \lred^* \true \\
%    Predicate(E, (\lamt x S T), f) & = & 
%    \forall x:STLCTerm.\judgeS {} {Base(S) \wedge Predicate(S,x) \rightarrow (Predicate(T,f~x)) \\
%    \\
%  \end{eqnarray*}
}



==> chapters/lambdah/figures/logicalrelation.tex <==

\renewcommand{\bisim}{\ensuremath{\sim}}
\renewcommand{\judgesimty}[3]{\ensuremath{#1\vdash #2\,\bisim\,#3}}

% The untyped version.  Just as useful, but uglier and less canonical
\renewcommand{\judgesim}[3]{\ensuremath{#1\vdash #2\,\bisim\,#3}}
% a hackish version used in proofs
\renewcommand{\judgesimmt}[2]{\ensuremath{{#1} \bisim {#2}}}

\newcommand{\extensionalequivalence}{
  \[
  \begin{array}{@{\qquad}lcl}  
    \multicolumn{3}{@{}l}{\mbox{ \fbox{$\judgesimt \env {\e_1} {\e_2 : T}$}~~ (defined by induction
        on $\Base {T}$) }} \\~\\
    \judgesimt \env {\e_1} {\e_2:\predty x B \predp} 
    & \defiff &
    \judgeIn \env {\e_1} {\predty x B \predp}
    \\ & &
    \judgeIn \env {\e_2} {\predty x B \predp}
    \\ & &
    \forall \closingsubst $ such that $ \judge {} \closingsubst \env, ~
    %\\ & &
    (\closingsubst(\e_1) \lred^* \constant) \Leftrightarrow (\closingsubst(\e_2) \lred^* \constant) 
    \\
    \\
    \judgesimt \env {\f_1} {\f_2 : {\plamt x S T}} 
    & \defiff &
    \forall \e_1, \e_2 $ such that $ \judgesimt \env {\e_1} {\e_2:S},
    \\ & & 
    \judgesimt \env {\f_1~\e_1} {\f_2~\e_2 : {\subst x {\e_1} {}}\, T \curlywedge \subst x {\e_2} {}\, T}
    \\
    
    \multicolumn{3}{@{}l}{\mbox{ \fbox{$S \curlywedge T$}}}
    \\~\\
    \predty x B \predp \curlywedge \predty x B \predq & \defeq & \predty x B {\predp \wedge \predq}
    \\
    \\
    \plamt x {S_1} {S_2} \curlywedge \plamt x {T_1} {T_2} & \defeq & \lamt x {(S_1 \curlywedge T_1)} {(S_2 \curlywedge T_2)}
    \\
  \end{array}
  \]
}


==> chapters/lambdah/figures/syntax.tex <==

% Basic syntax of lambda-H without casts
\newcommand{\basicsyntax}{
  \[
  \begin{array}{llr}
    \mydefhead {\e,\tmd,\tmf,\g,\predq,\predp ::=\qquad\qquad\qquad\qquad\qquad} {Terms:} 
    \mydefcase \constant                                                         {constant} 
    \mydefcase x                                                                 {variable} 
    \mydefcase {\lam x \tyS \e}                                                  {abstraction} 
    \mydefcase {\tmf~\e}                                                         {application} 
    \\
    \mydefhead{\val ::=\qquad\qquad\qquad\qquad\qquad}{Values: ($\subset$ Terms)}
    \mydefcase{\constant                              }{constant} 
    \mydefcase{\lam{x}{\tyS}{\e} 		                }{abstraction} 
    \\
    \mydefhead {\tyS,\tyT,\tyU::=}    {Types:} 
    \mydefcase {\lamt x \tyS \tyT}    {\bf \emph{dependent function type}}
    \mydefcase {\predty x B \predp}   {\bf \emph{refined basic type}}
  \end{array}
  \]
}



==> chapters/lambdah/figures/typerules.tex <==

% Type rules for lambda-H without casts.
\newcommand{\basictyperules}{
  \headtrule{$\judge \env \e T$}{\underline{T}ype rules}
  \begin{trules}
    \trule{T-Var}{
      (x:T)\in \env
    }{
      \judge \env x \tyT
    }
    
    \trule{T-Prim}{
    }{
      \judge \env \constant {\fun{ty}(\constant)}
    }
    
    \trule{T-Fun}{
      \judgeT{\env}{S} 
      \and
      \judge{\env,x:S}{\e}{\tyT}
    }{
      \judge{\env}{(\lam{x}{\tyS}{\e})}{(\lamt{x}{\tyS}{\tyT})}
    }
    
    \trule{T-App}{
      \judge \env \tmf {(\lamt{x}{\tyS}{\tyT})} 
      \and
      \judge \env \e \tyS 
    }{
      \judge \env {\app \tmf \e} {{\subst x \e {}}\, \tyT}
    }

    \trule{T-Sub}{
      \judge \env \e \tyS 
      \and
      \judgesub \env \tyS \tyT 
      \and
      \judgeT \env \tyT
    }{
      \judge \env \e \tyT
    }
  \end{trules}
}
 
\newcommand{\lambdahtypewellformedness}{ 
  \headtrule{$\judgeT \env \tyT$}{\underline{W}ell-formed \underline{t}ypes}
  \begin{trules}
    \trule{WT-Arrow}{
      \judgeT \env \tyS 
      \and 
      \judgeT {\env,x:S} \tyT
    }{
      \judgeT \env {\lamt x \tyS \tyT}
    }

    \trule{WT-Base}{
      \judge {\env,x:B} \predp \Bool	
    }{
      \judgeT \env {\predty x B \predp}
    }
  \end{trules}
}
 
\newcommand{\lambdahenvwellformedness}{ 
  \headtrule{$\judgeE{\env}$}{\underline{W}ell-formed \underline{e}nvironment}
  \begin{trules}
    \trule{WE-Empty}{\qquad\qquad }{
      \judgeE \emptyset
    }
    
    \trule{WE-Ext}{
      \judgeE \env 
      \and
      \judgeT \env T
    }{
      \judgeE {\env,x:T}
    }
  \end{trules}
}
  
\newcommand{\lambdahsubtyping}{ 
  \headtrule{$\judgesub{\env}{S}{T}$}{\underline{S}ubtyping}
  \begin{trules}
    \trule{S-Arrow}{
      \judgesub \env {\tyT_1}{\tyS_1}
      \and
      \judgesub{\env,x:\tyT_1}{\tyS_2}{\tyT_2}
    }{
      \judgesub \env {(\lamt x {\tyS_1} {\tyS_2})} {(\lamt x {\tyT_1}{\tyT_2})}
    }
    \\
    
    \trule{S-Base}{
      \judgeimp {\env,x:B} \predp \predq
    }{
      \judgesub \env {\predty x B \predp} {\predty x B \predq}
    }
  \end{trules}
}

\newcommand{\implicationrules}{
  \headtrule{$\judgeimp \env \predp \predq$}{Implication}
  \begin{trules}
    \trule{Imp}{
      \forall \sigma. \mbox{ if } \judge {} \sigma \env 
      \mbox{ and } \sigma(\predp) \lred^* \true
      \mbox{ then } \sigma(\predq) \lred^* \true
    }{
      \judgeimp \env \predp \predq
    }
  \end{trules}
  
  \headtrule{$\judge {} \sigma \env$}{Closing Substitution}
  \begin{trules}
    \trule{Subst}{
      \forall (x:T) \in \env,~
      \sigma(x) 
      \in \meaningf{\sigma(T)}
    }{
      \judge {} \sigma \env
    }
  \end{trules}
}



==> chapters/oldbackground/main-background.tex <==

\label{chapter:background}

This dissertation is best enjoyed with a strong background in
programming languages, especially type systems. Atop this foundation,
there stand four important research trends contributing to this work,
each dedicated a full section below: dynamic contracts, extended
static checking, refinement types, and soft typing. Discussion of
ongoing related work, some of which is the continuation of the
following background material, is deferred until
\hhref{Chapter}{chapter:relatedwork} so that it may be integrated into a
prospective view of the field. A viable reading strategy is to proceed
to the following substantive chapters and return here for references
to background material as needed.

\section{Types and Programming Languages}
\label{section:background:types}

The fundamental techniques of programming language theory that form
the basic background setting for this dissertation include:
operational semantics, denotational semantics, axiomatic semantics,
type systems (particularly dependent type systems), and logical
relations. 

For operational semantics and type systems, \citet{pierce_types_2002}
provides a thorough introduction in a textbook setting, using notation
and terminology similar to that of this dissertation. Its
sequel, \citet{pierce_advanced_2004}, covers advanced topics such as
logical relations, dependent types, and pure type systems.

From axiomatic semantics \citep{floyd_assigning_1967,
  hoare_axiomatic_1969, dijkstra_discipline_1976} we draw upon many
  descriptive terms for predicates that may be true of program
  fragments such as \emph{preconditions} (predicates that must hold
  before a procedure is begun), \emph{postconditions} (predicates that
  must hold after a procedure completes), \emph{invariants}
  (predicates that must always hold), \emph{weakest preconditions}
  (the weakest predicate that allows a fragment to complete
  successfully), and \emph{strongest postconditions} (the strongest
  predicate a fragment ensures).
\citet{winskel_formal_1993} is a suitable textbook for a unified
presentation.

\section{Dynamic Contracts}
\label{section:background:contracts}

\emph{Dynamic contracts} -- executable specifications written in the programming language
at hand -- 
have been incorporated into many languages, including
Turing \citep{holt_turing_1988}, Anna
\citep{luckham_programming_1990}, Eiffel \citep{meyer_eiffel:_1992},
Sather \citep{stoutamire_sather_1996}, Blue \citep{kolling_blue_1996},
JML~\citep{burdy_overview_2005, leavens_design_2006} and Spec\#
\citep{barnett_spec_2005}. In these languages, functions may have
precondition checks (executed before the body of the function is
evaluated), postcondition checks (executed after the result of the
function has been computed), and invariants (executed when a data
structure is modified, to ensure its integrity). The prior work of
most fundamental relevance is \citet{findler_contracts_2002} which
raised dynamic contracts to higher-order programming, providing some
of the technical approaches for enforcement which we build
upon. Higher-order contracts are also the subject of ongoing research,
dicussed in Chapter~\ref{chapter:relatedwork}.

\section{Extended Static Checking}
\label{section:background:esc}

While all of the above languages considered contracts to be predicates
written in the programming language at hand and executed at
appropriate moments during run-time, 
\citet{parnas_technique_1972}
and \citet{dijkstra_discipline_1976} 
proposed contracts written in a
non-executable formal logic. Multiple systems have used these as the
basis for static verification. For example,
PVS~\citep{rushby_subtypes_1998} 
featured full verification of logical
predicates via subtyping, while full verification of JML program
specifications built upon axiomatic semantics is implemented by
ESC/Java~\citep{flanagan_extended_2002}. As mentioned in the
introduction, the number of false positives was high, and this
dissertation may be viewed as directly inspired by that limitation,
but focused on providing a new theoretical foundation for the next
generation of practical tools.

\section{Refinement Types}
\label{section:background:refinementtypes}

The term \emph{refinement type} is not an agreed-upon mathematical
term, but an intuitive term applied to a variety of systems where the
basic types of a language may be ``refined'' to classify a more
precise subset of the terms of the language.  

It originated with
\citet{freeman_refinement_1991}, which proposed recursively defined
subsets of ML types, followed by \citet{hayashi_logic_1993},
\citet{denney_refinement_1998}, \citet{xi_dependent_1999},
\citet{xi_imperative_2000}, and \citet{davies_intersection_2000},
\citet{mandelbaum_effective_2003}, and
\citet{dunfield_tridirectional_2004}, each proposing a type
system incorporating various decidable logics, such as solutions of
linear inequalities of the integers and constraints in first-order
linear logic for imperative features. 
A general property that all of
these type systems share is that the language of types is deliberately
restricted to ensure that specifications can always be checked
statically.

In addition to limitations to ensure decidability, many properties are
expressed in an indirect style via \emph{indexed types} where only
special index values may be constrained. For example, a list of length
$n$ may be given the type $\t{list}(n)$, while a list of length
greater than $n$ may be given the type $\exists m>n, \t{list}(m)$ and
the integrity properties of more complex data structures such as
binary search trees must be encoded in terms of constraints on each
node\footnote{\hhref{Chapter}{chapter:relatedwork} surveys recent work on
the connection between global properties of a data structure and
specifications of its constructors}. We are concerned with the problem of allowing a programmer to
express properties in a direct style, such as $\predty x {\t{List}}
{\t{length}(x) > n}$ and $\predty x {\t{Tree}}
{\t{isBinarySearchTree}(x)}$ (a syntax chosen for its intuitive
similarity to set comprehension, explained fully in
Chapter~\ref{chapter:lambdah}) while still effectively enforcing at
least some portion of the specification statically.

\section{Soft Typing}
\label{section:background:softtyping}

\emph{Soft typing} \citep{fagan_soft_1991, wright_practical_1994,
  aiken_soft_1994} refers to the use of type systems technology in the
context of a dynamically typed language. Broadly, static type systems
reject any program that \emph{may} violate a precondition, while soft
type systems only reject programs that \emph{must} violate a
precondition.  The additional type information inferred during this
analysis may be used to remove some precondition checks that are part
of the normal functioning of the runtime of a dynamically typed
language. The techniques of Chapter~\ref{chapter:htc} and
Chapter~\ref{chapter:sage} resemble a form of soft typing, and as such
it forms a part of the relevant research context, though we work in
the tradition of static type systems, and are interested in allowing
programmers to express and enforce \emph{more} precise
specifications. Soft typing is closely related to \emph{gradual
  typing}, a field developed in parallel with the current work,
discussed in Chapter~\ref{chapter:relatedwork}.



==> chapters/sage/figures/castinsert.tex <==

\newcommand{\sagecastinsertionrules}{
  \headtrule{$\judgec \env \d \e T$}{\underline{C}ast Insertion rules}
  \begin{trules}
    \trule{C-Var}{
      (x:T) \in \env \mbox{~~~or~~~}
      (x=\e:T) \in \env
    }{
      \judgec \env x x {\predty y T {~y=x}}
    }

    \trule{C-Prim}{
    }{
      \judgec \env \constant \constant {\fun{ty}(\constant)}
    }

    \trule{C-Fun}{
      \judgecc \env \tyS {\tyS'} \type
      \and
      \judgec {\env,x:S'} \e {\e'} T
    }{
      \judgec \env {(\lam x S \e)} {(\lam x {S'} {\e'})} {(\lamt x {S'} T)}
    }
    
    \trule{C-Arrow}{
      \judgecc \env S {S'} \type
      \and
      \judgecc {\env,x:S'} T {T'} {} \type
    }{
      \judgec \env {(\funtyd x S T)} {(\funtyd x {S'} {T'})} \type
    }

    \trule{C-App1}{
      \judgec \env \f {\f'} \tyU
      \and
      \fun{unrefine}(\tyU) = \lamt x S T
      \and
      \judgecc \env \e {\e'} S
    }{
      \judgec \env {\f ~ \e} {\f' ~ \e'} {{\subst x {\e'} {}} \, T}
    }

    \trule{C-App2}{
      \judgecc \env \f {\f'} {(\Funty \dynamic \dynamic)}\\
      \judgecc \env \e {\e'} {\dynamic}  \\
    }{
      \judgec \env {\f ~ \e} {\f' ~ \e'} \dynamic
    }

    \trule{C-Let}{
      \judgecc \env S {S'} \type \\
      \judgecc \env \val {\val'} {S'} \\ 
      \judgec {\env,(x=\val':S')} \e {\e'} T 
    }{
      \judgec {\env ~} {~ \letexpt x \val S \e ~} {~ \letexpt x {\val'} {S'} {\e'} ~} {~ \subst x {\val'} {}\, T'}
    }
  \end{trules}
}

\newcommand{\sagecheckingrules}{
  \headtrule{$\judgecc \env \d \e \tyT$}{\underline{C}ast Insertion and \underline{C}hecking rules}
  \begin{trules}
    \trule{CC-Ok}{
      \judgec \env \tmd \e S \\
      \judgesubalg \pyes \env S T 
    }{
      \judgecc \env \tmd \e T
    }
    
    \trule{CC-Chk}{
      \judgec \env \tmd \e S\qquad
      \judgesubalg \pmaybe \env S T
    }{
      \judgecc \env \tmd {({\cast T} \, \e)} T
    }
  \end{trules}
}


==> chapters/sage/figures/evalrules.tex <==

\newcommand{\sageevalrules}{
  \[
  \begin{array}{@{}rcl@{}r}
    \headrule{$\tmd \red \e$}{Redex \underline{E}valuation}
    \app {(\lam{x}{S}{\e})} \val &\red& \subst x \val {} \, \e &\rel{E-App} \\
    \letexpt x \val S \e &\red& \subst x \val {} \, \e &\rel{E-Let} \\
    \deltadeftss{{\cal S}[\sagefix~U~\val]}{{\cal S}[\app{\val}{({\sagefix}~U~{v})}]}{\rel{E-Fix}}
    \deltadeftss{\t{if}_{T}~\true~\val_1~\val_2} {\val_1~\t{unit}}{\rel{E-If1}}
    \deltadeftss{\t{if}_{T}~\false~\val_1~\val_2} {\val_2~\t{unit}}{\rel{E-If2}}
    \\
    \headrule{${\tmd}\lred{\e}$}{\underline{E}valuation}
    \cbvctx[\d] &\lred& \cbvctx[\e] \quad \mbox{if $\d\red \e$} & \rel{E-Compat} 
    \\
    \\
    \headrule{\tmctx, \tyctx}{Call-by-value Contexts}
    \multicolumn{4}{l}{
      \begin{array}{lll}
        \cbvctx  & ::= &
        ~\hole
        ~|~ \app \cbvctx \e
        ~|~ \app \val \cbvctx
        \hole
        ~|~ \app \tmctx \e
        ~|~ \app \e \tmctx
        ~|~ \lam x \tyS \tmctx
      \end{array}
    }
    \\
    \\
    \headrule{\cal S}{Unfolding Contexts}
    \multicolumn{4}{l}{
      \begin{array}{lll}
        \cal S &::=&
        ~\app \hole \val
        ~|~ \cast \hole ~ \val
      \end{array}
    }
    \\
    \\
    \headrule{\tmctx, \tyctx}{Arbitrary Contexts}
    \multicolumn{4}{l}{
      \begin{array}{lll}
        \tmctx &::=&
        ~\hole 
        ~|~ \tmctx ~ \e 
        ~|~ \e ~ \tmctx
        ~|~ \lamt x \tmctx T
        ~|~ \lamt x S \tmctx
        ~|~ \lam x \tmctx \e
        ~|~ \lam x S \tmctx
        \\
        &&
        ~|~ \letexpt x \tmctx S \e
        ~|~ \letexpt x \e \tmctx \e
        ~|~ \letexpt x \e S \tmctx
      \end{array}
    }
  \end{array}
  \]
}

\newcommand{\sagecastevalrules}{
  \[
  \begin{array}{@{}rcl@{}r}
    \headrule{${\tmd}\red{\e}$}{Redex \underline{E}valuation}
    \deltadeftss{\cast \dynamic ~ v}{v}{\rel{E-Cast-Dyn}}
    \deltadeftss{\cast \constant ~ \val}{\val}{\rel{E-Cast-Basic}} 
    \multicolumn{4}{c}{\mbox{\qquad if for $\constant \in \setz{\Int,\Bool,\Unit}$ and appropriate $\val$}} \\
    \\
    \deltadeftss{ \cast {\funtyd x S T} ~ \val }{ \lam x S {\cast T ~ (v~(\cast D ~ x))}       }{ \rel{E-Cast-Fn} }
    \multicolumn{3}{r}{\mbox{where $D=\fun{domain}(v)$}} \\
    \\
    \deltadeftss{
      \cast {\Refine~T~\f} ~ \val
    }{
      \t{Checking} ~ T ~ f ~ \val ~ (f~(\cast T ~ \val))
    }{
      \rel{E-Cast-Begin}
    }
    \deltadeftss{
      \t{Checking} ~ T ~ f ~ \val ~ \true
    }{
      \cast T ~ \val
    }{
      \rel{E-Cast-End}
    }
    \\
    \deltadeftss{\cast \type ~ v}{v}{\rel{E-Cast-Type}}
    \multicolumn{4}{c}{\mbox{\qquad if $v$ is of one of the forms $\Int,\Bool,\Unit,\dynamic,\type,\lamt x S T, \t{Refine}~T~f$}}
  \end{array}
  \]

  {\ssp
  \begin{eqnarray*}
    \fun{domain}                                   & : & \fun{Value} \rightarrow \fun{Term} \\
    \fun{domain}(\lam x T \e)                      & = & T \\
    \fun{domain}(\t{fix}~(\funtyd x T {T'})~\val)  & = & T \\
    \fun{domain}(\constant~\val_1\dots \val_{i-1}) & = & \mbox{type of $i^{th}$ argument to $\constant$}
  \end{eqnarray*}
  }
}


==> chapters/sage/figures/syntax.tex <==

\newcommand{\sagesyntax}{
  \[
  \begin{array}{llr}
    \mydefhead{\d,\e,\f,\g,\predp,\predq,\tyS,\tyT,\tyU ::=\qquad\qquad\qquad}{Terms:} 
    \mydefcase{x                        }{variable} 
    \mydefcase{\constant                }{primitive} 
    \mydefcase{\letexpt x \e S \e       }{binding} 
    \mydefcase{\lam{x}{S}{\e}           }{abstraction} 
    \mydefcase{\f~\e                    }{application} 
    \mydefcase{\funtyd{x}{S}{T}         }{function type}
  \end{array}
  \]

  \[
  \begin{array}{llr}
    \mydefhead{u,v,V,W ::=\qquad\qquad\quad\quad}{Values} 
    \mydefcase{\lam x S \e                  }{abstraction} 
    \mydefcase{\funtyd x S T                }{function type}
    \mydefcase{\constant                    }{primitive} 
    \mydefcase{\constant~v_1~\dots~v_n      }{primitive, $0<n<\fun{arity}(\constant)$} 
    \mydefcase{\t{Refine}~W~v               }{refinement}
    \mydefcase{\t{fix}~W~v                  }{recursive type}
  \end{array}
  \]
}


==> chapters/sage/figures/typerules.tex <==

\newcommand{\sagetyperules}{
  \[
  \begin{array}{llr}
    \mydefhead{\env::=}{Environments:} 
    \mydefcase{\emptyset                       }{empty environment}
    \mydefcase{\env,x:T                        }{environment extension}
    \mydefcase{\env,x=\val:T\qquad\qquad       }{environment term extension}
  \end{array}
  \]

  \headtrule{$\judgeE \env$}{\underline{W}ell-formed \underline{e}nvironment}
  \begin{trules}
    \trule{We-Empty}{
    }{
      \judgeE \emptyset
    }
    
    \trule{We-Ext1}{
      \judgeE \env \\
      \judge \env T \type         
    }{
      \judgeE {\env,x:T}
    }
    
    \trule{We-Ext2}{
      \judgeE \env \\
      \judge \env T \type \\
      \judge \env \e T
    }{
      \judgeE {\env,x:T=\e}
    }
  \end{trules}

  \headtrule{$\judge \env \e T$}{\underline{T}ype rules}
  \begin{trules}
    \trule{T-Const}{
    }{
      \judge{\env}{\constant}{\fun{ty}(\constant)}
    }

    \trule{T-Var}{
      (x:T)\in \env \mbox{~~~or~~~}
      (x=\val:T)\in \env
    }{
      \judge{\env}{x}{\predty{y}{T}{~y=x}}
    }

    \trule{T-Fun}{
      \judge{\env}{S}{\type} \\
      \judge{\env,x:S}{\e}{T}
    }{
      \judge \env {(\lam x S \e)} {(\funtyd x S T)}
    }
    
    \trule{T-Arrow}{
      \judge \env S \type \\
      \judge {\env,x:S} T \type
    }{
      \judge \env {(\funtyd x S T)} \type
    }

    \trule{T-App}{
      \judge \env \f {(\funtyd x S T)} \\
      \judge \env \e S 
    }{
      \judge \env {\f ~ \e} {\subst x \e {} \, T}
    }

    \trule{T-Let}{
      \judge \env \val S \\
      \judge {\env,(x=\val:S)}{\e}{T} 
    }{
      \judge \env {\letexpt x \val S \e} {\subst x \val {}\, T}
    }

    \trule{T-Sub}{
      \judge{\env}{\e}{S}\\
      \judgesub{\env}{S}{T} 
    }{
      \judge{\env}{\e}{T}
    }
  \end{trules}
}

